GPU-CFR: 80x Faster Counterfactual Regret Minimization by Compiling the Game to Static Dataflow and CUDA Graph Replay

Counterfactual regret minimization (CFR) is one of the few large numerical workloads that still runs faster on CPUs than on GPUs. Each iteration sweeps a game tree with up to billions of states in millions of small, interdependent gather and scatter steps issued through a generic tree interface. On a GPU every kernel finishes in microseconds, so kernel launches and framework dispatch dominate the run time, and prior GPU implementations have lost to optimized CPU code. We observe that for a fixed game, everything about a CFR iteration except the numerical values is known before the first iteration runs. We propose GPU-CFR, a compiler and runtime built on this observation. It compiles any game once into static dataflow: flat edge and information-set arrays, precomputed indices, and depth-level batched passes fix the entire operation sequence, and only solver state changes between iterations. Static chance folding, depth-level execution blocks, and a dual-lane reach buffer cut the number of framework operations by up to 18.1x. Because shapes, indices, and buffer addresses never change, CUDA Graph Replay records the iteration once and replays it with a single graph launch. On one A100, across an eight-game suite that spans card games, dice games, and board games, GPU-CFR runs 29.8--80.4x faster than the fastest prior GPU CFR on the same accelerator, and 14--258x faster than LiteEFG, one of the fastest open-source CPU implementations, on the four largest games. The compiled representation carries most of that margin: on eight CPU threads with no accelerator it is already 2.2--51.1x faster than the GPU baseline. On the CPU the optimized path reproduces the reference iterates bitwise, and tree construction and graph capture pay for themselves within the first solve. GPU-CFR beats every CPU and GPU baseline on the mid-to-large games of the suite without changing the update rule.

==> figures/TABLE_T17_derived.tex <==
\begin{table*}[!htb]
\centering
\caption{Derived speedups behind every range and median quoted in the text, computed
from the unrounded per-game medians of \cref{tab:matrix} (shown here to three
significant figures, ms per iteration). Ranges in the text are the minimum and
maximum of a column over the eight games, or over the four largest (the last four
rows) where stated; medians are over the eight games.}
\label{tab:derived}
{
\setlength{\tabcolsep}{3.5pt}
\begin{tabular}{lrrrrrrrrrrr}
\toprule
Game & graph & eager & CPU & Kim & LiteEFG & Kim/graph & Kim/eager & Kim/CPU & CPU/graph & LiteEFG/graph & eager/graph \\
\midrule
Kuhn & 0.113 & 0.401 & 0.177 & 9.057 & 0.008 & 80.449 & 22.595 & 51.114 & 1.574 & 0.075 & 3.560 \\
Dark Hex 2x2 & 0.174 & 0.536 & 0.243 & 11.691 & 0.065 & 67.156 & 21.827 & 48.128 & 1.395 & 0.373 & 3.077 \\
HUNL river & 0.210 & 0.411 & 1.697 & 9.642 & 16.857 & 45.898 & 23.464 & 5.680 & 8.080 & 80.243 & 1.956 \\
Leduc & 0.304 & 0.738 & 0.612 & 12.860 & 1.233 & 42.265 & 17.432 & 21.002 & 2.012 & 4.053 & 2.425 \\
Goofspiel-5 & 0.245 & 0.591 & 0.765 & 13.180 & 3.375 & 53.835 & 22.289 & 17.233 & 3.124 & 13.785 & 2.415 \\
HUNL turn & 0.397 & 0.617 & 5.360 & 11.893 & 102.160 & 29.978 & 19.285 & 2.219 & 13.512 & 257.508 & 1.554 \\
Liar's Dice & 0.556 & 0.933 & 4.378 & 16.545 & 102.880 & 29.772 & 17.740 & 3.779 & 7.877 & 185.131 & 1.678 \\
Battleship & 0.380 & 0.688 & 3.138 & 14.393 & 80.952 & 37.837 & 20.905 & 4.586 & 8.250 & 212.809 & 1.810 \\
\bottomrule
\end{tabular}}
\end{table*}


==> figures/latex_includes.tex <==
% Auto-collected include snippets for the paper figures.
% Regenerate figures via figures/run_all.sh after the gated campaign lands.
%
% STALE: this file is not \input by main.tex. The live figure environments and
% captions are in paper/sections/*.tex. Numbers below may be out of date; do not
% copy from here without checking the live captions and the generated tables.

% === F1 hero: scaling (main body, §1/§6.2) ===
\begin{figure}[t]
    \centering
    \includegraphics[width=0.72\textwidth]{figures/fig1_hero_scaling.pdf}
    \caption{Steady-state time per CFR iteration as a function of game
    size (log--log; lower is better). Below ${\sim}10^3$ nodes the single-thread C++
    baseline (LiteEFG) is fastest --- GPU launch overhead dominates. Beyond $10^5$
    nodes GPU-CFR's compiled, CUDA-graph-replayed iteration is up to ${\sim}500\times$
    faster than single-thread LiteEFG and 3--4 orders of magnitude faster than
    OpenSpiel's Python CFR, while producing bitwise-identical iterates to a reference
    implementation under the same CFR variant. Baselines are research frameworks, not
    hand-optimized CPU solvers (\S\ref{sec:setup}).}
    \label{fig:hero}
\end{figure}

% === F-arch (Fig 2, MANUAL/TikZ): one-iteration dataflow (main body, §4) ===
% [MANUAL] drawn as TikZ directly in the paper source (sections/method fig).

% === F2 ladder: optimization ladder (main body, §6.3) ===
\begin{figure}[t]
    \centering
    \includegraphics[width=0.85\textwidth]{figures/fig2_ladder.pdf}
    \caption{Left: per-iteration time on the 434k-node HUNL turn subgame (A100,
    float32) for the reference eager implementation, the compiled depth-level
    dataflow, and the same dataflow replayed as a CUDA graph. Right: PyTorch/Aten
    operations issued per iteration (load-immune count). All three variants produce
    bitwise-identical regrets after 22 iterations.}
    \label{fig:ladder}
\end{figure}

% === F3 graph-vs-eager per game (appendix) ===
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/fig3_graph_ablation.pdf}
    \caption{CUDA-graph replay vs.\ eager execution: steady-state ms per CFR$^+$
    iteration for every game in the suite (log scale). Labels give the eager/graph
    ratio. CUDA graphs remove per-kernel launch and dispatcher overhead; they do not
    fuse the iteration into a single kernel.}
    \label{fig:graphablation}
\end{figure}

% === F4 convergence curves (main body, §6.4) ===
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\textwidth]{figures/fig4_curves.pdf}
    \caption{Exploitability vs.\ training wall-clock (log--log) on the four games all
    backends support. Curves compare time-to-quality across systems; per-iteration
    quality is not comparable across frameworks because CFR variants differ
    (\S\ref{sec:discussion}).}
    \label{fig:curves}
\end{figure}

% === F5 HUNL curves (main body, §6.5) ===
\begin{figure}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{figures/fig5_hunl_curves.pdf}
    \caption{Convergence on the native HUNL subgames (GPU-CFR only; no baseline supports
    these trees). Exploitability is exact-best-response based, in units of the game's
    chip payoffs.}
    \label{fig:hunlcurves}
\end{figure}

% === F6 scaling sweep (main body, §6.2) ===
\begin{figure}[t]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/fig6_scaling.pdf}
    \caption{Scaling past the default suite: HUNL turn subgames with $K$ hands per
    player (tree size grows ${\sim}K^2$). Solid: steady-state ms/iteration (CUDA
    graph). Dashed: achieved bandwidth implied by an approximate bytes-moved model,
    against the A100's ${\sim}2$\,TB/s peak.}
    \label{fig:scaling}
\end{figure}

% === Tables (input directly) ===
% \input{figures/TABLE_T1_suite.tex}     — main body §5
% \input{figures/TABLE_T2_matrix.tex}    — main body §6.1
% \input{figures/TABLE_T3_opcount.tex}   — appendix (summary numbers quoted in §6.3)
% \input{figures/TABLE_T4_memory.tex}    — appendix
% \input{figures/TABLE_T6_overhead.tex}  — main body §6.6 (or appendix)


==> sections/7_discussion.tex <==
\section{Systems Implications}
\label{sec:discussion}

\paragraph{Algorithmic semantics define the unit of comparison.}
CFR variant, update order, and averaging convention jointly determine the iterates
\cite{burch2019revisiting}
and the work performed by one iteration, so systems timing must hold them matched
(\cref{tab:convergence}).

\paragraph{Static execution changes the runtime bottleneck.}
Compilation moves topology, indexing, and scheduling to build time; graph
replay then turns the fixed kernel sequence into one graph launch. Launch cost is
fixed per iteration, so the compiled schedule absorbs additional parallel work at
constant submission cost, so the margin grows with scale.

